Scalar auxiliary variable finite element scheme for the parabolic-parabolic Keller-Segel model

We describe and analyze a finite element numerical scheme for the parabolic-parabolic Keller-Segel model. The scalar auxiliary variable method is used to retrieve the monotonic decay of the energy associated with the system at the discrete level. This method relies on the interpretation of the Keller-Segel model as a gradient flow. The resulting numerical scheme is efficient and easy to implement. We show the existence of a unique non-negative solution and that a modified discrete energy is obtained due to the use of the SAV method. We also prove the convergence of the discrete solutions to the ones of the weak form of the continuous Keller-Segel model.

==> commands.tex <==
\newcommand\ind[1]{   {1\hspace{-1.2mm}{\rm I}}_{\{#1\} }    }
\newcommand{\wt}[1] {{\widetilde #1}}
\newcommand{\commentout}[1]{}
%
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Sp}{\mathbb{S}}
%
\newcommand {\al} {\alpha}
\newcommand {\e}  {\varepsilon}
\newcommand {\es}{\epsilon}

\newcommand {\da} {\delta}
\newcommand {\sg} {\sigma}
\newcommand {\vp} {\varphi}
\newcommand {\lb} {\lambda}
\newcommand {\Lb} {\Lambda}
\newcommand {\Chi} {{\bf \raise 2pt \hbox{$\chi$}} }
%
\newcommand {\dt}   {\Delta t}
\newcommand {\sgn} { {\rm sgn} }
\newcommand {\dv}  { {\rm div} }
%
\newcommand {\cae} { {\mathcal E} }
\newcommand {\cah} { {\mathcal H} }
\newcommand {\car} { {\mathcal R} }
\newcommand {\cas} { {\mathcal S} }
\newcommand {\caL} { {\mathcal L} }
%
\newcommand {\f}   {\frac}
\newcommand {\p}   {\partial}
\newcommand {\pp}   {{\prime \prime}}
\newcommand {\ov}  {\overline}
%
\newcommand{\dis}{\displaystyle}
%
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea} {\begin{array}{rl}}
\newcommand{\eea} {\end{array}}
\newcommand{\bepa}{\left\{ \begin{array}{l}}
\newcommand{\eepa} {\end{array}\right.}
%

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\parent}[1]{\left(#1\right)}
\newcommand{\fespace}{V_h}
%
%\newcommand{\dis}{\displaystyle}
%\newcommand {\proof} {\noindent {\bf Proof}. }
%
\newcommand*{\dd}{\mathop{\kern0pt\mathrm{d}}\!{}}
\newcommand{\ndiffeps}{\left(n_{h,\epsilon}^{k+1}-n_{h,\epsilon}^k\right)}
\newcommand{\ndiffepssp}{n_{h,\epsilon}^{k+1}-n_{h,\epsilon}^k}
\newcommand{\seconde}{{\prime\prime}}
\newcommand{\psipenkk}{\psi^{\prime}_{+,\epsilon}(n^{k+1}_{h,\epsilon})}
\newcommand{\psipmk}{\psi^{\prime}_{-}(n^{k}_{h,\epsilon})}

\newcommand{\scal}[2]{\left(#1 , #2\right)}
\newcommand{\lscal}[2]{\left(#1 , #2\right)}

\newcommand{\bas}{\phi}

\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}

\renewcommand{\u}{u}
\newcommand{\nn}{n}

\newcommand{\kk}{{k+1}}
\newcommand{\heps}{{h,\epsilon}}
\newcommand{\peps}{{+,\epsilon}}
\newlength\eqnspace
\eqnspace = 1.4em

%%%%%%%%%%%%%%%%%%%%%%%

==> results.tex <==
\section{Numerical results}
\subsection{1D numerical results}
The table \ref{tab:parameter1D} summarizes the parameters used in the one dimensional numerical scheme. The initial cell density is a uniform distributed random perturbation around the value $u^0$.
\begin{table}
	\centering
	\begin{tabular}{|c|c|}
		\hline 
		&Parameters  \\
		\hline
		$\Delta t$& $0.001$\\
		$\Delta x$ & $0.1$  \\
        $u^0$ & $0.5$\\
        $\chi_c/D_u$ & $40$ \\
        $\alpha$ & $0.5$\\
        $\delta$ & $1$\\
		$\epsilon$ & $0.01$\\
		$\tau$ & $0.01$\\
		\hline
    \end{tabular}
    \caption{Parameters of the 1D test case}
	\label{tab:parameter1D}
\end{table}


\begin{figure}
	\centering
	\includegraphics[scale = 0.36]{Images/1D_mass_0-5_begin.png}
	\includegraphics[scale = 0.36]{Images/1D_mass_0-5_mid.png}
	\includegraphics[scale = 0.36]{Images/1D_mass_0-5_end.png}
	\caption{Solution $u_h$ at $3$ different times with $u^0=0.5$.}
	\label{fig:sol3steps-0.5}
\end{figure}

\begin{figure}[h!!]
	\centering
	\includegraphics[scale = 0.6]{Images/Energy-1D.png}
	\caption{Evolution of the modified energy through time.}
	\label{fig:energy}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale = 0.6]{Images/c_h-end-mass-0-5.png}
	\caption{Concentration of chemo-attractant at steady state.}
	\label{fig:c_h-1D}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale = 0.6]{Images/rn-1D.png}
	\caption{Evolution of the scalar variable $r$ through time.}
	\label{fig:rn-1D}
\end{figure}

